Polarization-Tuned Fano Resonances in All-Dielectric Short-Wave Infrared Metasurface

The short-wave infrared (SWIR) is an underexploited portion of the electromagnetic spectrum in metasurface-based nanophotonics despite its strategic importance in sensing and imaging applications. This is mainly attributed to the lack of material systems to tailor light-matter interactions in this range. Herein, we address this limitation and demonstrate an all-dielectric silicon-integrated metasurface enabling polarization-induced Fano resonance control at SWIR frequencies. The platform consists of a two-dimensional Si/GeSn core/shell nanowire array on a silicon wafer. By tuning the light polarization, we show that the metasurface reflectance can be efficiently engineered due to Fano resonances emerging from the electric and magnetic dipoles competition. The interference of optically induced dipoles in high-index nanowire arrays offers additional degrees of freedom to tailor the directional scattering and the flow of light while enabling sharp polarization-modulated resonances. This tunability is harnessed in nanosensors yielding an efficient detection of 10^{-2} changes in the refractive index of the surrounding medium.

==> space_saving_tricks.tex <==
%% Make everything look better.
%% http://tex.stackexchange.com/questions/553/what-packages-do-people-load-by-default-in-latex
%% http://www.howtotex.com/packages/9-essential-latex-packages-everyone-should-use/
\usepackage{microtype}

%% Shrink space around figures.
%% This beats manually adding negative \vspace commands everywhere.
\setlength{\textfloatsep}{0pt}
\setlength{\textfloatsep}{20pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{10pt plus 2pt minus 4pt}
\setlength{\textfloatsep}{10pt plus 1pt minus 2pt}
\setlength{\dbltextfloatsep}{3pt}
\setlength{\intextsep}{5pt}
\setlength{\abovecaptionskip}{5pt}
% \setlength{\belowcaptionskip}{3pt}
\setlength{\parskip}{4pt}
%% around equations
\setlength{\abovedisplayskip}{3pt}
\setlength{\belowdisplayskip}{3pt}
\setlength\abovedisplayshortskip{3pt}
\setlength\belowdisplayshortskip{3pt}


%% The wrapfigure environment is also a good way to use less space for a small figure.
%% It is finicky.
%% See: http://en.wikibooks.org/wiki/LaTeX/Floats,_Figures_and_Captions#Wrapping_text_around_figures

%% Shrink space around enumerate and itemize
%% From: http://tex.stackexchange.com/questions/10684/vertical-space-in-lists
\usepackage{enumitem}
%% Set it globally:
\setlist{nosep} % or \setlist{noitemsep} to leave space around whole list
\setlist{itemsep=1pt, topsep=3pt}
%% Or locally:
% \begin{enumerate}[itemsep=1pt, topsep=12pt, partopsep=0pt]

%% Less space around titles.
%% From: http://tex.stackexchange.com/questions/4999/change-whitespace-above-and-below-a-section-heading
%\usepackage[medium,compact]{titlesec}
%% or
%\usepackage{titlesec}
%\titlespacing*{\section}{0pt}{*1}{*1}

%% Shrink the \paragraph command.
\renewcommand{\paragraph}[1]{\noindent {\bf #1}}

%% Allow Latex to use a smaller minimum spacing between lines.
%\renewcommand{\baselinestretch}{0.97}
%\renewcommand{\baselinestretch}{0.982}

%% Shrink space between lines. You probably want to prefer baselinestretch in general.
%% From: http://tex.stackexchange.com/questions/23824/6-lines-in-one-inch
%% 6 lines in one inch with an 11pt font:
%\linespread{0.901}
%\linespread{0.909}
%\linespread{1}

%% Shrink the spacing between lines in just the bibliography. This is good.
\usepackage{setspace}

%% Then wrap the bibliography in a \begin{spacing}. You can wrap any section like this.
% \begin{spacing}{0.9}
% \bibliographystyle{...}
% \bibliography{references}
% \end{spacing}
